$\nu$-DBA: Neural Implicit Dense Bundle Adjustment Enables Image-Only Driving Scene Reconstruction

The joint optimization of the sensor trajectory and 3D map is a crucial characteristic of bundle adjustment (BA), essential for autonomous driving. This paper presents $\nu$-DBA, a novel framework implementing geometric dense bundle adjustment (DBA) using 3D neural implicit surfaces for map parametrization, which optimizes both the map surface and trajectory poses using geometric error guided by dense optical flow prediction. Additionally, we fine-tune the optical flow model with per-scene self-supervision to further improve the quality of the dense mapping. Our experimental results on multiple driving scene datasets demonstrate that our method achieves superior trajectory optimization and dense reconstruction accuracy. We also investigate the influences of photometric error and different neural geometric priors on the performance of surface reconstruction and novel view synthesis. Our method stands as a significant step towards leveraging neural implicit representations in dense bundle adjustment for more accurate trajectories and detailed environmental mapping.

==> introduction.tex <==
\section{Introduction}

Building a dense map of the driving scene is desirable for autonomous vehicles, aiding localization, planning, and simulation. Bundle adjustment (BA) is indispensable for this reconstruction task when using images with noisy trajectories, which jointly optimizes camera poses and map points. However, the sparse images and small parallax angles along the driving route make dense surface mapping challenging using only images and noisy trajectories in driving scenes.
%Despite promising performance have been achieved based on LiDAR scans, jointly optimizing the 

%and a back-end optimizes previous sensor poses and, eventually, the 3D map \cite{di2023photometric}. A good back-end is important for the SLAM system to improve the accuracy of bundle adjustment (BA) and reconstruction maps. SLAM systems are widely used in autonomous driving, robotics, and more. In this paper, we focus on the back-end of the SLAM system for driving scenes, which is more challenging than other applications because of fewer input views.

% Traditional SLAM systems build sparse point cloud maps due to limited computing power. These systems use the RGB inputs directly \cite{2016Direct} or sparse feature point cloud maps \cite{mur2015orb} for bundle adjustment. The former, called direct method, is affected by illumination changes, while the latter, called feature-based method, is limited by the lack of features. Both optimization methods suffer from drift due to the lack of strong features such as surface constraints.

To investigate this problem, we delve into BA from the perspectives of \textit{map parametrization} and \textit{measurement metric}, respectively. 
The most popular BA methods take sparse 3D scene points cloud as the map parametrization, as shown in Fig. \ref{teaser} (a). This representation is consistent across different views, yet falls short in describing the dense geometry. Nevertheless, these sparse BA methods provide insights into the measurement metric. There are two types of measurement metrics in sparse BA:
%We begin from the existing mature sparse BA, which has two lines of measurement metrics: 
geometric error and photometric error. COLMAP \cite{schoenberger2016sfm} and photometric BA \cite{alismail2017photometric} are two representative works, respectively. 
%Both lines of works employ sparse 3D scene points cloud as the map parametrization. 
Geometric BA utilizes the scene point correspondence across images for optimization, while photometric BA utilizes the local patch consistency of the scene point projections. In \cite{campos2021orb}, geometric BA is shown to be more accurate than photometric BA, which might be induced by sensitivity in illumination and calibration.

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth,trim=4 4 4 4,clip]{images/paper/teaser0316.png}
\caption{\textbf{Comparison of BA methods.} (a) Traditional geometric sparse BA with 3D point map. (b) Geometric dense BA with 2D keyframes. (c) Photometric dense BA with the neural implicit surface. (d) \textbf{$\mathbf{\nu}$-DBA}: geometric dense BA with the neural implicit surface.

} 
\label{teaser}
\end{figure}


In recent years, dense BA has received increasing attention. A representative work, DROID-SLAM~\cite{teed2021droid}, parametrizes the dense map based on a set of 2D keyframes and their optimizable depth maps, as shown in Fig. \ref{teaser} (b). A dense map can be obtained by projecting the depth maps to 3D. However, keyframe depth might be redundant in 3D, and there are no 3D consistency constraints to enforce the overlap part to be the same, which may limit the accuracy of the resultant map. Despite the limitation in the map parameterization, DROID-SLAM inherits the advantage of geometric BA, as it can be essentially considered as geometric BA by employing dense optical flow using RAFT~\cite{teed2020raft} as the measurement. This makes DROID-SLAM a geometric dense BA (DBA), as the scene points correspondence in geometric sparse BA is akin to sparse optical flow.

Recent advances in neural implicit representation have achieved impressive high-fidelity novel view synthesis~\cite{mildenhall2021nerf} and scene reconstruction~\cite{wang2021neus, Yu2022MonoSDF}. With the differentiable rendering, the image regression loss can be back-propagated to learn the 3D representation~\cite{wang2021neus, Yu2022MonoSDF}.  Considering such neural mapping from the perspective of dense BA, we find that the neural implicit representation acts as a 3D dense map parametrization, avoiding the consistency issue of keyframe depth maps. The differentiable rendering can be viewed as a photometric error-based measurement model,
%\yl{why is it photometric BA? it does not "utilize local patch consistency of scene point projection" as defined above}
yielding a photometric dense BA, as shown in Fig. \ref{teaser} (c). Utilizing such a photometric dense BA as the back-end, several neural implicit representation-based SLAM systems are proposed~\cite{zhu2022nice, zhu2023nicer, johari2022eslam, mao2023ngel, zhang2023goslam}. Despite some of them are applicable to RGB images for indoor scenes~\cite{zhu2023nicer,zhang2023goslam}, existing methods in this direction struggle in street scenes with RGB input, indicating that street scenes pose challenges due to complex illumination and textureless regions. This raises a question: \textit{Can we bridge the 3D neural implicit representation with the geometric error to improve the dense BA accuracy?}


%In feature-based sparse BA, 3D scene representation performs better than 2D keyframe depth since the 3D scene representation is more consistent. As a result, we would like to find a 3D scene representation for dense BA.

%used sparse point cloud maps due to limited computing power. According to the optimization method, these methods can be categorized into direct methods \cite{2016Direct} and feature-based (indirect) methods. Direct methods, such as DSO-SLAM \cite{2016Direct}, define an objective function over photometric error and use the images directly for optimization. However, direct methods are sensitive to illumination changes and are less robust to geometric distortion. Feature-based methods, such as ORB-SLAM \cite{mur2015orb} and Colmap \cite{schoenberger2016sfm}, overcome these limitations by extracting features from images first. The camera position and scene geometry are computed as a function of these feature observations. However, feature-based methods only use part of the image, called sparse BA, which is limited when lacking features.

Following the idea, in this paper, we propose $\nu$-DBA (pronounced as ``neuDBA''), a geometric dense BA framework with 3D neural implicit surface as map parametrization, which optimizes both the map surface and trajectory poses using geometric error derived from dense flow, as illustrated in Fig. \ref{teaser} (d). 
% To simplify expression, we will refer to geometric dense bundle adjustment with 3D neural implicit surface as \textbf{$\nu$-DBA} in the following paper. 
Apart from the framework, we investigate the effectiveness of photometric error and other neural geometric prior on the quality of the surface reconstruction and the novel view synthesis. Moreover, to relieve the generalization gap of the flow prior, we further propose to fine-tune the flow model through per-scene self-supervision. In the experiments, we evaluate our method on several driving scene datasets and demonstrate superior trajectory and mapping accuracy. In summary, we make the following contributions:
\begin{itemize}
\item We propose a geometric error-based dense BA framework with 3D consistent representation i.e. neural implicit surface as the map parametrization, for driving scene reconstruction.

\item We propose to self-supervise the optical flow model to narrow the generalization gap, which further improves the quality of the reconstructed surface.

%\item For optimization, we provide a comparison of choices of using photometric loss directly and using geometry cues extracted from images, including monocular geometry cues and correspondence geometry cues.

\item We evaluate the framework on several driving scene datasets, demonstrating superior performance in reconstruction and trajectory optimization, and investigating the effect of photometric error and other neural geometric priors.
\end{itemize}

==> method_old.tex <==
Given a sequence of RGB images $\{I_0, I_1, \dots,I_k\}$ with preprocessed camera poses $\{T_1,T_2,\dots,T_k\}$, our method can extract dense and complete surfaces. As illustrated in Fig.\ref{overview}, our pipeline can be divided into three main parts: (1) Correspondence Geometry Estimation. Our method first inference the geometry of the scene by a matching network that can be self-supervised for per-scene optimization. (2) Neural implicit scene representation. We then leverage a multi-range network to represent the scene and train it with the given RGB images and geometry evaluation results.

\subsection{Correspondence Geometry Evaluation} \label{cge}

Accurate geometric priors, such as LiDAR data, play a crucial role in the rapid training of neural implicit scene representation. However, in the cases without LiDAR data, we should infer the geometry information from the RGB image inputs. Unlike \cite{Yu2022MonoSDF} and \cite{guo2023streetsurf}, we choose optical flow and stereo estimated by unimatch \cite{xu2023unifying} instead of monocular geometric cues to guide the optimization process. Compared with monocular geometry prediction which performs on every single frame, flow and stereo estimation perform on different frames, making them geometrically continuous. Furthermore, as the flow estimation model can be self-supervised with only RGB image inputs, we can finetune an estimation model for each scenario.

\subsubsection{Optical Flow}
Optical flow finds the 2D-pixel displacement field between two images, which can be easily obtained via an off-the-shelf flow estimator. We use the pretrained unimatch model to estimate the optical flow $F_i$ for each input frame pair $\{I_{i}, I_{i+1}\}$. Compared with monocular depth which is a relative cue, the optical flow is an absolute scale that can be directly used to supervise the scene representation model.

\subsubsection{Stereo Matching}
Stereo matching is the process of finding the pixels in the multiscopic views that correspond to the same 3D point in the scene. The unimatch model estimates the disparity between a given stereo pair $I^l_{i}, I^r_{i}$. The accuracy of stereo matching is often higher than that of optical flow, but can only be used in scenes with stereo pair.



\subsection{Implicit Scene Representation} \label{isr}
Since we aim to tackle the unbounded task in outdoor scenes, similar to \cite{barron2022mipnerf360, kaizhang2020}, we leverage a two-part model including a close-range model and a distant model. The close-range model represents the objects tens of meters away from the camera, while the distant model represents the scene hundreds or even thousands of meters away from the camera and the sky.

\subsubsection{Close-Range Model} 

The close-range model represents the geometry as a signed distant function (SDF). Given a 3D point $\mathbf{x}$, it returns the point's distance to the closest surface $\hat{s}$. The RGB color $\hat{\mathbf{c}}$ of the given point $\mathbf{x}$ and a view direction $\mathbf{v}$ is also predicted by the close-range model. Therefore, we can define the function of SDF value $\mathcal{S}$ and color $\mathcal{C}$

\begin{equation}
[\hat{s}, \mathbf{z}] = \mathcal{S}_\theta(\mathbf{x}), \quad
\hat{\mathbf{c}} = \mathcal{C}_\theta(\mathbf{v}, \mathbf{z})
\label{close model}
\end{equation}
 As shown in Fig.\ref{pipeline}, the whole close-range model consists of three parts: a 3D hash table as the feature grid and two small MLPs as the decoders. The feature vector $\mathbf{z}$ is the output of the geometry decoder of the SDF model and $\theta$ is the network weights.

\subsubsection{Distant Model}

To handle unbounded scenes, we leverage scene parameterization the same as \cite{guo2023streetsurf}. To form a 4D input, we sample on cuboid shells and apply inverse cuboid warping. Samples of the distant-view model lie on cuboid shells. The cuboid shells are scaled proportionally from the cuboid shell of the close-range space with inverse-proportionally increasing scales. The warped point $\mathbf{x}'$ of the sample $\mathbf{x}$ on the $i$th cuboid shell can be expressed as 

\begin{equation}
\mathbf{x}'=\left[r_i\mathbf{x}, r_i\right], \quad r_i=\frac{1}{(1-i/n)+(i/n)(1/r_{max})}
\label{inverse}
\end{equation}
where $n$ is the number of cuboid shells and $r_{max}$ is the scale of the largest cuboid shell relative to the close-range shell. The distant model is a hyper 4D hash table. Given the 4D input, the network directly outputs the density $\hat{\sigma}$ and RGB color $\hat{\mathbf{c}}$ of the sample point.

\subsection{Volume Rendering}
Following recent work \cite{mildenhall2021nerf}, we optimize our model with 2D supervision using volume rendering. Given camera intrinsic parameters and current camera pose, we cast a ray $\mathbf{r}$ from the camera center $\mathbf{o}$ through the pixel along its normalized view direction $\mathbf{v}$. We sample $N$ points along a ray, denoted as $\mathbf{x}_i = \mathbf{o} + d_i\mathbf{v}$, where $d_i$ is the depth of point $\mathbf{x}_i$, and $i \in {1,\cdots, N}$. The points can be divided into close-range points $\mathbf{x}_i^c$ and distant points $\mathbf{x}_i^d$, that query the different scene models. 

For close-range points $\mathbf{x}_i^c$, the close-range model predicts the SDF values $\hat{s}_i^c$ and color values $\hat{\mathbf{c}}_i^c$. Following NeuS \cite{wang2021neus}, we convert the SDF values into density values ${\sigma_i^c}$. For distant points $\mathbf{x}_i^d$, the distant model predicts the density values $\sigma_i^d$ and color values $\hat{\mathbf{c}}_i^d$. Then, we can render the color $\hat{C}$ and depth $\hat{D}$ for the given ray $\mathbf{r}$ via numerical integration

\begin{equation}
\hat{D}(\mathbf{r}) = \sum_{i=1}^N T_i\alpha_i d_i \quad \text{and} \quad \hat{\mathbf{C}}(\mathbf{r}) = \sum_{i=1}^N T_i\alpha_i \mathbf{c}_i
\label{render}
\end{equation}
where
\begin{equation}
 \quad T_i = \prod_{j=1}^i(1-\alpha_j) \quad \text{and} \quad \alpha_i = 1-\exp(-\sigma_i\delta_i)
\label{render}
\end{equation}

Unlike other methods, our method uses optical flow as a supervision which means we should also render the optical flow. We can also obtain the optical flow by volume rendering. Given a image pair $\{I_k,I_j\}$ and a ray $\mathbf{r}_j$ of the pixel $\mathbf{p}_j$ in image $I_j$, we can calculate the pixel location of every sample $\mathbf{x}^{\mathbf{r}_j}_i$ on the ray $\mathbf{r}_j$ on another image via differentiable homography in \cite{yao2018mvsnet}

\begin{equation}
H(d)=K_kR_k\left(I-\frac{(R_k^{-1} \mathbf{t}_k-R_j^{-1}\mathbf{t}_j)\mathbf{n}^\top_jR_j}{d}\right)R_j^{-1}K_j^{-1}
\label{homo}
\end{equation}
that $\{K_j, R_j, \mathbf{t}_j\}$ is the camera intrinsics, rotations and translations of frames $\{I_j\}$, $\mathbf{n}$ is the principle axis of the reference camera, and $d$ is the depth of point in reference view $I_j$. Then, we can get the pixel location of sample $\mathbf{x}^{\mathbf{r}_j}_i$ on image $I_k$: $\mathbf{p}^i_k \sim H(d_i)\cdot\mathbf{p}_j$ where '$\sim$' denotes the projective equality. The optical flow $\hat{\mathbf{F}}$ of pixel $\mathbf{p}_j$ from frame $I_j$ to frame $I_k$ can be calculated as 
\begin{equation}
\hat{\mathbf{F}}(\mathbf{r}_j) = \sum_{i=1}^N T_i\alpha_i \mathbf{p}^i_k - \mathbf{p}_j
\label{render}
\end{equation}


\subsection{Optimization}

\subsubsection{Self-supervised Optical Flow Model Optimization}
As mentioned in \ref{cge}, the optical flow model can be self-supervised without using any information, e.g. poses, except RGB image inputs. Since our task is a per-scene optimization task, following \cite{long2022sparseneus}, the inference result of the optical flow model can be improved by a per-scene fine-tuning process. Following \cite{jonschkowski2020matters}, we use census loss, smoothness loss, and self-supervision loss to optimize the optical flow model. 

\subsubsection{Scene Representation Optimization and Bundle Adjustment}
For scene representation optimization, we first use 2D supervision with a simple photometric loss and optical flow loss.

\begin{equation}
\mathcal{L}_{p}=\sum_{\mathbf{r}\in R}\|\hat{\mathbf{C}}(\mathbf{r})-{\mathbf{C}}(\mathbf{r})\|_2, \quad
\mathcal{L}_{f}=\sum_{\mathbf{r}\in R}\|\hat{\mathbf{F}}(\mathbf{r})-{\mathbf{F}}(\mathbf{r})\|_2
\label{color loss}
\end{equation}

If a stereo pair is given, we can calculate the estimated disparity with the rendering depth and supervise the model with disparity loss

\begin{equation}
\mathcal{L}_{d}=\sum_{\mathbf{r}\in R}\|\hat{D}_{disp}(\mathbf{r})-{D}_{disp}(\mathbf{r})\|_2, \quad D_{disp} = \frac{f\cdot b}{D}
\label{depth loss}
\end{equation}
where $f$ is the focal length, $b$ is the baseline, $D_{disp}$ is the disparity map and $D$ is the depth map.

Following common practice, we also add an Eikonal term on the sampled points to regularize SDF values in 3D space and sparsity loss to penalize the uncontrollable free surfaces:

\begin{equation}
 \mathcal{L}_{eik}=\sum_{\mathbf{x}\in \mathcal{X}}(\|\nabla \mathcal{S}_\theta(\mathbf{x})\|_2-1)^2 
\label{eik}
\end{equation}
\begin{equation}
 \mathcal{L}_{spa}=\sum_{\mathbf{x}\in \mathcal{X}}\exp(-\tau\cdot\|\mathcal{S}_\theta(\mathbf{x})\|) 
\label{eik}
\end{equation}
where $\tau$ is a hyperparameter to rescale the SDF value. 

To eliminate ambiguous occupancy of the close-range and distant-view models, an entropy regularization term is added
\begin{equation}
 \mathcal{L}_{ent}=f_{ent}(\hat{O}_c(\mathbf{r})), \quad f_{ent}(x)=-(x\ln x+(1-x)\ln(1-x))
\label{eik}
\end{equation}
where $\hat{O}_c(\mathbf{r})$ is the opacity of close range model along ray $\mathbf{r}$ that can be calculate as $\hat{O}_c(\mathbf{r}) = \sum_{i=1}^N T^c_i\alpha^c_i$.

The overall loss we use to optimize our implicit scene representation is:

\begin{equation}
 \mathcal{L}=\mathcal{L}_{p}+\lambda_1\mathcal{L}_{f}+\lambda_2\mathcal{L}_{d}+\lambda_3\mathcal{L}_{eik}+\lambda_4\mathcal{L}_{spa}+\lambda_5\mathcal{L}_{ent}
\label{loss}
\end{equation}

To simultaneously optimize the camera poses, we conduct a bundle adjustment (BA) with Eq. \ref{loss}, where we also include the optimization of the scene representation as well as the extrinsic $T$ of the cameras.

\subsection{Road Surface Initialization} \label{rsi}
As discussed in \cite{guo2023streetsurf}, the disentanglement of close-range and distant-view models is an unsupervised and ill-posed problem with almost no constraints. The road surface initialization, in which the close-range SDF model is pre-trained to have a zero-level set that is roughly aligned with the road surface, is important to address the issue in the driving scenes. To get the road surface, we leverage the corresponding information provided by the estimated optical flow. The corresponding points are triangulated with the preprocessed camera poses to obtain a 3D point cloud. Then, we find the plane with the largest support in the point cloud using RANSAC. The fitting plane is used to initialize the close-range SDF model.


\subsection{Voxel-based Sampling}
The sampling strategy is important for neural implicit field training. Recent works \cite{muller2022instant,mao2023ngel, long2022sparseneus, guo2023streetsurf} have proved that the octree structure can significantly improve sampling efficiency. As a result, we employ the octree to sample points along the rays in the close-range model. The octree is first initialized by the triangulated point cloud in subsection \ref{rsi} and is continuously updated as the close-range model training. We uniformly sample $N$ points per voxel the ray hits. To further improve the sampling efficiency, we discard those sampling points whose SDF value is higher than the threshold after $60\%$ of the total number of training iterations. These sampling strategies make sure our sampling points are close to the surface.
